Moby: Empowering 2D Models for Efficient Point Cloud Analytics on the Edge

3D object detection plays a pivotal role in many applications, most notably autonomous driving and robotics. These applications are commonly deployed on edge devices to promptly interact with the environment, and often require near real-time response. With limited computation power, it is challenging to execute 3D detection on the edge using highly complex neural networks. Common approaches such as offloading to the cloud induce significant latency overheads due to the large amount of point cloud data during transmission. To resolve the tension between wimpy edge devices and compute-intensive inference workloads, we explore the possibility of empowering fast 2D detection to extrapolate 3D bounding boxes. To this end, we present Moby, a novel system that demonstrates the feasibility and potential of our approach. We design a transformation pipeline for Moby that generates 3D bounding boxes efficiently and accurately based on 2D detection results without running 3D detectors. Further, we devise a frame offloading scheduler that decides when to launch the 3D detector judiciously in the cloud to avoid the errors from accumulating. Extensive evaluations on NVIDIA Jetson TX2 with real-world autonomous driving datasets demonstrate that Moby offers up to 91.9% latency improvement with modest accuracy loss over state of the art.

==> discussion.tex <==
\section{Discussion and Limitations}
\label{sec:discussion}

\noindent\textbf{Occlusion in Images.}
\label{sec:occlusion}
Although \sys brings significant latency gain to running 3D object detection models, we notice that the accuracy performance of \sys still has room to improve. 
One problem that haunts existing image-based 3D object detection and also \sys is the occlusion in 2D images \cite{arnold2019survey, qian20223d}.
As we know, an important characteristic of driving environment is occlusion or truncation present in crowded scenes where vehicles can block the view of other agents and themselves \cite{arnold2019survey}.
Since 2D-to-3D transformation in \sys is based on the visual perception of images, its accuracy is likely to be affected by the occlusion effect.
A possible solution is to integrate an occlusion reasoning module into \sys to handle object missing.
While our system can dramatically reduce latency with minor accuracy loss, we have not investigated how much occlusion affects our system's performance, which is a promising direction for \sys to advance its performance in the future. 

\noindent\textbf{Generalization to Other Classes.}
\label{sec:other_classes}
While \sys is mainly evaluated on the 3D detection task of cars, it can be generalized to other 3D detection tasks, such as pedestrians and cyclists. For these tasks, minor design modification is needed in the 2D-to-3D transformation module to estimate the bounding box accurately. 
For example, because pedestrians and cyclists are smaller than cars, their object centers can be simply calculated by averaging the value of all points in the point cluster.
Other task-specific design for the pipeline is also needed to maximize its benefit.
We expect \sys achieves similar performance gains in these scenarios, as it can be applied similarly to leverage 2D models for 3D object detection to accelerate inference.
We leave this part as future work.
